KATch: A Fast Symbolic Verifier for NetKAT

We develop new data structures and algorithms for checking verification queries in NetKAT, a domain-specific language for specifying the behavior of network data planes. Our results extend the techniques obtained in prior work on symbolic automata and provide a framework for building efficient and scalable verification tools. We present KATch, an implementation of these ideas in Scala, featuring an extended set of NetKAT operators that are useful for expressing network-wide specifications, and a verification engine that constructs a bisimulation or generates a counter-example showing that none exists. We evaluate the performance of our implementation on real-world and synthetic benchmarks, verifying properties such as reachability and slice isolation, typically returning a result in well under a second, which is orders of magnitude faster than previous approaches. Our advancements underscore NetKAT's potential as a practical, declarative language for network specification and verification.

==> Makefile <==
FILE = pldi24

# DIFF_COMMIT ?= 6a4e39fb40c05d45599fcca35337088389ff5d54 # Old commit: 27 Oct
# DIFF_COMMIT ?= df67474fd9ee333e6c91cc5d33efb5094375e7f0 # Submission version: 17 Nov
DIFF_COMMIT ?= eeca0c41397603a3f9208b0335c89d65822ebec8 # Phase 2 submission: 24 Mar

THIS_REPO ?= git@github.com:GaloisInc/5stars.git

PAPER_DIR ?= writeups/pldi24
UNDO_PAPER_DIR ?= ../..

build:
	latexmk -pdf -auxdir=aux $(FILE)

clean:
	latexmk -c -auxdir=aux
	rm -f *.bbl

.PHONY: build clean

diff:
	rm -rf tmp/diff
	rm -rf tmp/old-src
	mkdir -p tmp/diff/old
	mkdir -p tmp/diff/new
	mkdir -p tmp/diff/delta
	
	make build
	latexpand $(FILE).tex > tmp/diff/new/$(FILE).tex
	cp *.csv tmp/diff/new/
	cp *.bib tmp/diff/new/
	cp *.sty tmp/diff/new/
	
	git clone --depth=1 $(THIS_REPO) tmp/old-src
	cd tmp/old-src && ( \
	  git fetch origin $(DIFF_COMMIT) && \
	  git checkout $(DIFF_COMMIT) && \
	  cd $(PAPER_DIR) && ( \
	    latexmk -pdf -auxdir=aux $(FILE) && \
	    latexpand $(FILE).tex > $(UNDO_PAPER_DIR)/../diff/old/$(FILE).tex && \
	    cp *.csv $(UNDO_PAPER_DIR)/../diff/old/ && \
	    cp *.bib $(UNDO_PAPER_DIR)/../diff/old/ && \
	    cp *.sty $(UNDO_PAPER_DIR)/../diff/old/    \
	))
	
	cd tmp/diff/new && ( \
	  latexdiff ../old/$(FILE).tex $(FILE).tex > ../delta/$(FILE).tex && \
	  cp *.csv ../delta/ && \
	  cp *.bib ../delta/ && \
	  cp *.sty ../delta/ \
	)
	
	cd tmp/diff/delta && ( \
	  (latexmk -pdf -auxdir=aux -interaction=nonstopmode $(FILE).tex || true) \
	)
	
	cp tmp/diff/delta/$(FILE).pdf $(FILE)-diff.pdf



==> phase2-plots/Fig10_table.tex <==
\begin{tabular}{llrrrr}
\toprule
Name & Type & Size & KATch (s) & Frenetic (s) & Speedup \\
\midrule
Layer42 & reachability & 135 & 0.00 & 0.05 & 18 \\
Layer42 & unreachability & 135 & 0.00 & 0.04 & 14 \\
Layer42 & slicing & 142 & 0.01 & 0.07 & 13 \\
Compuserv & unreachability & 539 & 0.01 & 0.35 & 55 \\
Compuserv & reachability & 539 & 0.01 & 0.35 & 53 \\
Compuserv & slicing & 554 & 0.01 & 0.81 & 59 \\
Airtel & reachability & 786 & 0.01 & 0.83 & 65 \\
Airtel & unreachability & 786 & 0.01 & 0.82 & 69 \\
Airtel & slicing & 802 & 0.03 & 1.98 & 71 \\
Belnet & reachability & 1388 & 0.02 & 3.18 & 169 \\
Belnet & unreachability & 1388 & 0.02 & 3.20 & 173 \\
Belnet & slicing & 1412 & 0.04 & 7.99 & 181 \\
Shentel & reachability & 1865 & 0.01 & 3.90 & 278 \\
Shentel & unreachability & 1865 & 0.02 & 3.96 & 243 \\
Shentel & slicing & 1894 & 0.04 & 9.76 & 248 \\
Arpa & unreachability & 1964 & 0.02 & 4.23 & 199 \\
Arpa & reachability & 1964 & 0.02 & 4.23 & 201 \\
Arpa & slicing & 1994 & 0.06 & 10.42 & 185 \\
Sanet & unreachability & 4100 & 0.03 & 23.54 & 859 \\
Sanet & reachability & 4100 & 0.03 & 23.30 & 768 \\
Sanet & slicing & 4144 & 0.07 & 62.21 & 917 \\
Uunet & reachability & 5456 & 0.05 & 81.03 & 1666 \\
Uunet & unreachability & 5456 & 0.05 & 80.67 & 1482 \\
Uunet & slicing & 5506 & 0.15 & 203.80 & 1339 \\
Missouri & unreachability & 9680 & 0.07 & 165.59 & 2411 \\
Missouri & reachability & 9680 & 0.11 & 168.15 & 1576 \\
Missouri & slicing & 9748 & 0.22 & 441.72 & 1992 \\
Telcove & reachability & 10720 & 0.10 & 441.47 & 4559 \\
Telcove & unreachability & 10720 & 0.07 & 441.46 & 6586 \\
Telcove & slicing & 10792 & 0.25 & 1121.30 & 4464 \\
Deltacom & reachability & 26978 & 0.22 & 2210.27 & 10137 \\
Deltacom & unreachability & 26978 & 0.20 & 1964.41 & 9721 \\
Deltacom & slicing & 27092 & 0.48 & 5098.57 & 10556 \\
Cogentco & unreachability & 79682 & 0.59 & 18926.65 & 31892 \\
Cogentco & reachability & 79682 & 0.62 & 18894.99 & 30241 \\
Cogentco & slicing & 79880 & 1.54 & 54247.73 & 35212 \\
\bottomrule
\end{tabular}


==> plots/Flip_comparison_table.tex <==
\begin{tabular}{lrrrr}
\toprule
Name & Size (KB) & KATch (s) & Frenetic (s) & Speedup \\
\midrule
flip1 & 0.13 & 0.00 & 0.04 & 11 \\
flip2 & 0.23 & 0.00 & 0.04 & 11 \\
flip3 & 0.33 & 0.00 & 0.03 & 8 \\
flip4 & 0.43 & 0.00 & 0.04 & 10 \\
flip5 & 0.53 & 0.00 & 0.05 & 13 \\
flip6 & 0.62 & 0.01 & 0.14 & 27 \\
flip7 & 0.72 & 0.00 & 0.36 & 86 \\
flip8 & 0.82 & 0.01 & 1.88 & 294 \\
flip9 & 0.92 & 0.01 & 7.01 & 1260 \\
flip10 & 1.03 & 0.01 & 24.95 & 2111 \\
flip11 & 1.14 & 0.01 & 86.12 & 7340 \\
\bottomrule
\end{tabular}


==> plots/Flip_comparison_table_old.tex <==
\begin{tabular}{lrrrr}
\toprule
Name & Size & KATch (s) & Frenetic (s) & Speedup \\
\midrule
flip1 & 8 & 0.00 & 0.04 & 11 \\
flip2 & 15 & 0.00 & 0.04 & 11 \\
flip3 & 22 & 0.00 & 0.03 & 8 \\
flip4 & 29 & 0.00 & 0.04 & 10 \\
flip5 & 36 & 0.00 & 0.05 & 13 \\
flip6 & 43 & 0.01 & 0.14 & 27 \\
flip7 & 50 & 0.00 & 0.36 & 86 \\
flip8 & 57 & 0.01 & 1.88 & 294 \\
flip9 & 64 & 0.01 & 7.01 & 1260 \\
flip10 & 71 & 0.01 & 24.95 & 2111 \\
flip11 & 78 & 0.01 & 86.12 & 7340 \\
\bottomrule
\end{tabular}


==> plots/Full_reachability_comparison_table.tex <==
\begin{tabular}{llrrrr}
\toprule
Name & Type & Size (KB) & KATch (s) & Frenetic (s) & Speedup \\
\midrule
Arpanet196912 & reachability & 0.74 & 0.01 & 0.30 & 50 \\
Arpanet196912 & reachability & 0.74 & 0.01 & 0.30 & 45 \\
Renam & reachability & 0.96 & 0.00 & 0.53 & 140 \\
Renam & reachability & 0.96 & 0.01 & 0.53 & 84 \\
Mren & reachability & 1.29 & 0.00 & 1.11 & 231 \\
Mren & reachability & 1.29 & 0.01 & 1.11 & 122 \\
Telecomserbia & reachability & 1.36 & 0.00 & 0.97 & 245 \\
Telecomserbia & reachability & 1.36 & 0.01 & 0.97 & 102 \\
Epoch & reachability & 1.42 & 0.00 & 0.91 & 220 \\
Epoch & reachability & 1.42 & 0.01 & 0.91 & 98 \\
Layer42 & reachability & 1.42 & 0.01 & 1.11 & 204 \\
Layer42 & reachability & 1.42 & 0.01 & 1.11 & 124 \\
Napnet & reachability & 1.42 & 0.01 & 1.06 & 196 \\
Napnet & reachability & 1.42 & 0.01 & 1.06 & 118 \\
Basnet & reachability & 1.66 & 0.01 & 2.01 & 317 \\
Basnet & reachability & 1.66 & 0.02 & 2.01 & 118 \\
Nordu1989 & reachability & 1.66 & 0.01 & 1.93 & 326 \\
Nordu1989 & reachability & 1.66 & 0.01 & 1.93 & 146 \\
Dataxchange & reachability & 1.68 & 0.01 & 1.19 & 190 \\
Dataxchange & reachability & 1.68 & 0.01 & 1.19 & 130 \\
Sanren & reachability & 1.73 & 0.00 & 1.69 & 366 \\
Sanren & reachability & 1.73 & 0.01 & 1.69 & 125 \\
Padi & reachability & 1.78 & 0.01 & 7.57 & 1303 \\
Padi & reachability & 1.78 & 0.04 & 7.57 & 181 \\
Getnet & reachability & 1.79 & 0.00 & 1.82 & 390 \\
Getnet & reachability & 1.79 & 0.01 & 1.82 & 133 \\
Netrail & reachability & 1.92 & 0.01 & 2.06 & 293 \\
Netrail & reachability & 1.92 & 0.01 & 2.06 & 166 \\
Gblnet & reachability & 2.07 & 0.01 & 3.40 & 609 \\
Gblnet & reachability & 2.07 & 0.02 & 3.40 & 180 \\
Heanet & reachability & 2.11 & 0.01 & 2.20 & 408 \\
Heanet & reachability & 2.11 & 0.01 & 2.20 & 152 \\
HiberniaIreland & reachability & 2.14 & 0.01 & 3.35 & 582 \\
HiberniaIreland & reachability & 2.14 & 0.02 & 3.35 & 178 \\
Arpanet19706 & reachability & 2.65 & 0.01 & 5.17 & 385 \\
Arpanet19706 & reachability & 2.65 & 0.03 & 5.17 & 157 \\
Nordu2005 & reachability & 2.65 & 0.01 & 6.13 & 659 \\
Nordu2005 & reachability & 2.65 & 0.03 & 6.13 & 199 \\
Nsfcnet & reachability & 2.66 & 0.01 & 7.03 & 737 \\
Nsfcnet & reachability & 2.66 & 0.03 & 7.03 & 221 \\
Ai3 & reachability & 3.02 & 0.02 & 9.33 & 522 \\
Ai3 & reachability & 3.02 & 0.04 & 9.33 & 212 \\
Cesnet1993 & reachability & 3.02 & 0.01 & 9.44 & 1184 \\
Cesnet1993 & reachability & 3.02 & 0.03 & 9.44 & 315 \\
JanetExternal & reachability & 3.26 & 0.05 & 14.68 & 283 \\
Gridnet & reachability & 3.29 & 0.01 & 6.34 & 783 \\
Gridnet & reachability & 3.29 & 0.02 & 6.34 & 279 \\
Itnet & reachability & 3.57 & 0.01 & 18.80 & 1619 \\
Itnet & reachability & 3.57 & 0.04 & 18.80 & 459 \\
Singaren & reachability & 3.57 & 0.01 & 18.59 & 1954 \\
Singaren & reachability & 3.57 & 0.04 & 18.59 & 471 \\
Abilene & reachability & 3.83 & 0.05 & 12.78 & 273 \\
Abilene & reachability & 3.83 & 0.07 & 12.78 & 174 \\
Sprint & reachability & 4.09 & 0.01 & 14.61 & 1473 \\
Sprint & reachability & 4.09 & 0.04 & 14.61 & 396 \\
Globalcenter & reachability & 4.32 & 0.01 & 6.92 & 842 \\
Globalcenter & reachability & 4.32 & 0.02 & 6.92 & 327 \\
TLex & reachability & 4.50 & 0.01 & 28.18 & 2508 \\
TLex & reachability & 4.50 & 0.05 & 28.18 & 587 \\
Cesnet1999 & reachability & 4.81 & 0.01 & 38.99 & 3479 \\
Cesnet1999 & reachability & 4.81 & 0.06 & 38.99 & 656 \\
Cesnet1997 & reachability & 4.81 & 0.01 & 35.05 & 3150 \\
Cesnet1997 & reachability & 4.81 & 0.06 & 35.05 & 586 \\
Kreonet & reachability & 4.82 & 0.02 & 41.72 & 2592 \\
Kreonet & reachability & 4.82 & 0.06 & 41.72 & 732 \\
HiberniaCanada & reachability & 4.94 & 0.01 & 30.65 & 2649 \\
HiberniaCanada & reachability & 4.94 & 0.07 & 30.65 & 469 \\
Nsfnet & reachability & 5.01 & 0.02 & 31.40 & 1886 \\
Nsfnet & reachability & 5.01 & 0.05 & 31.40 & 580 \\
Eenet & reachability & 5.07 & 0.01 & 45.15 & 3818 \\
Eenet & reachability & 5.07 & 0.06 & 45.15 & 733 \\
Navigata & reachability & 5.14 & 0.02 & 37.02 & 2196 \\
Navigata & reachability & 5.14 & 0.06 & 37.02 & 668 \\
Nordu1997 & reachability & 5.50 & 0.02 & 70.83 & 4007 \\
Nordu1997 & reachability & 5.50 & 0.07 & 70.83 & 1061 \\
Ilan & reachability & 5.62 & 0.01 & 55.71 & 4718 \\
Ilan & reachability & 5.62 & 0.07 & 55.71 & 796 \\
Uninet & reachability & 5.65 & 0.01 & 38.85 & 2898 \\
Uninet & reachability & 5.65 & 0.06 & 38.85 & 668 \\
Compuserve & reachability & 5.76 & 0.02 & 62.47 & 2980 \\
Compuserve & reachability & 5.76 & 0.07 & 62.47 & 951 \\
Eunetworks & reachability & 5.91 & 0.02 & 51.63 & 3409 \\
Eunetworks & reachability & 5.91 & 0.09 & 51.63 & 581 \\
HiberniaUk & reachability & 6.29 & 0.01 & 66.54 & 4491 \\
HiberniaUk & reachability & 6.29 & 0.09 & 66.54 & 719 \\
Spiralight & reachability & 6.36 & 0.02 & 69.02 & 4306 \\
Spiralight & reachability & 6.36 & 0.09 & 69.02 & 798 \\
Claranet & reachability & 6.49 & 0.02 & 82.76 & 3743 \\
Claranet & reachability & 6.49 & 0.08 & 82.76 & 1068 \\
Nordu2010 & reachability & 6.75 & 0.13 & 133.85 & 1022 \\
Grena & reachability & 7.00 & 0.01 & 95.49 & 6479 \\
Grena & reachability & 7.00 & 0.11 & 95.49 & 835 \\
KentmanJul2005 & reachability & 7.13 & 0.02 & 114.01 & 5184 \\
KentmanJul2005 & reachability & 7.13 & 0.09 & 114.01 & 1203 \\
Garr199901 & reachability & 7.19 & 0.02 & 129.77 & 8377 \\
Garr199901 & reachability & 7.19 & 0.09 & 129.77 & 1397 \\
Marwan & reachability & 7.20 & 0.02 & 102.47 & 4492 \\
Marwan & reachability & 7.20 & 0.10 & 102.47 & 1025 \\
Rhnet & reachability & 7.20 & 0.02 & 114.55 & 5803 \\
Rhnet & reachability & 7.20 & 0.11 & 114.55 & 1062 \\
Peer1 & reachability & 7.33 & 0.02 & 120.67 & 4904 \\
Peer1 & reachability & 7.33 & 0.10 & 120.67 & 1258 \\
HostwayInternational & reachability & 7.39 & 0.02 & 108.01 & 6589 \\
HostwayInternational & reachability & 7.39 & 0.10 & 108.01 & 1053 \\
Nextgen & reachability & 8.08 & 0.03 & 140.05 & 5310 \\
Nextgen & reachability & 8.08 & 0.12 & 140.05 & 1143 \\
Fatman & reachability & 8.15 & 0.02 & 180.77 & 9506 \\
Fatman & reachability & 8.15 & 0.12 & 180.77 & 1556 \\
Airtel & reachability & 8.44 & 0.05 & 195.12 & 4153 \\
Airtel & reachability & 8.44 & 0.13 & 195.12 & 1515 \\
Sago & reachability & 8.69 & 0.02 & 163.82 & 8256 \\
Sago & reachability & 8.69 & 0.17 & 163.82 & 961 \\
Jgn2Plus & reachability & 8.69 & 0.03 & 227.89 & 8582 \\
Jgn2Plus & reachability & 8.69 & 0.15 & 227.89 & 1537 \\
Goodnet & reachability & 8.80 & 0.02 & 211.21 & 10395 \\
Goodnet & reachability & 8.80 & 0.11 & 211.21 & 1983 \\
HiberniaNireland & reachability & 9.01 & 0.02 & 209.54 & 10412 \\
HiberniaNireland & reachability & 9.01 & 0.14 & 209.54 & 1538 \\
Arpanet19719 & reachability & 9.01 & 0.04 & 195.82 & 4792 \\
Arpanet19719 & reachability & 9.01 & 0.16 & 195.82 & 1199 \\
Ibm & reachability & 9.14 & 0.02 & 223.49 & 11199 \\
Ibm & reachability & 9.14 & 0.12 & 223.49 & 1820 \\
BsonetEurope & reachability & 9.14 & 0.03 & 248.80 & 8811 \\
BsonetEurope & reachability & 9.14 & 0.12 & 248.80 & 2053 \\
Ans & reachability & 9.20 & 0.04 & 228.42 & 6090 \\
Ans & reachability & 9.20 & 0.13 & 228.42 & 1821 \\
Pacificwave & reachability & 9.36 & 0.03 & 300.00 & 10552 \\
Pacificwave & reachability & 9.36 & 0.12 & 300.00 & 2532 \\
Savvis & reachability & 9.72 & 0.02 & 255.55 & 11464 \\
Savvis & reachability & 9.72 & 0.16 & 255.55 & 1565 \\
Restena & reachability & 9.79 & 0.02 & 300.00 & 14409 \\
Restena & reachability & 9.79 & 0.14 & 300.00 & 2107 \\
Aarnet & reachability & 9.98 & 0.51 & 271.58 & 532 \\
Aarnet & reachability & 9.98 & 0.84 & 271.58 & 323 \\
Noel & reachability & 10.04 & 0.03 & 300.00 & 9437 \\
Noel & reachability & 10.04 & 0.14 & 300.00 & 2183 \\
Easynet & reachability & 10.30 & 0.02 & 300.00 & 13589 \\
Easynet & reachability & 10.30 & 0.15 & 300.00 & 1975 \\
Rediris & reachability & 10.50 & 0.04 & 300.00 & 7904 \\
Rediris & reachability & 10.50 & 0.14 & 300.00 & 2172 \\
Twaren & reachability & 10.61 & 0.02 & 300.00 & 14296 \\
Twaren & reachability & 10.61 & 0.15 & 300.00 & 1961 \\
Oxford & reachability & 11.00 & 0.03 & 300.00 & 8799 \\
Oxford & reachability & 11.00 & 0.17 & 300.00 & 1771 \\
Highwinds & reachability & 11.05 & 0.02 & 300.00 & 12038 \\
Highwinds & reachability & 11.05 & 0.14 & 300.00 & 2174 \\
Marnet & reachability & 11.07 & 0.06 & 300.00 & 5150 \\
Marnet & reachability & 11.07 & 0.17 & 300.00 & 1757 \\
EliBackbone & reachability & 11.25 & 0.02 & 300.00 & 12050 \\
EliBackbone & reachability & 11.25 & 0.16 & 300.00 & 1864 \\
Quest & reachability & 11.32 & 0.04 & 300.00 & 7890 \\
Quest & reachability & 11.32 & 0.16 & 300.00 & 1927 \\
BtAsiaPac & reachability & 11.33 & 0.04 & 300.00 & 7630 \\
BtAsiaPac & reachability & 11.33 & 0.16 & 300.00 & 1887 \\
Internetmci & reachability & 11.34 & 0.03 & 300.00 & 11357 \\
Internetmci & reachability & 11.34 & 0.14 & 300.00 & 2101 \\
Atmnet & reachability & 11.66 & 0.03 & 300.00 & 9509 \\
Atmnet & reachability & 11.66 & 0.23 & 300.00 & 1322 \\
GtsRomania & reachability & 11.80 & 0.02 & 300.00 & 12072 \\
GtsRomania & reachability & 11.80 & 0.20 & 300.00 & 1517 \\
Harnet & reachability & 11.87 & 0.02 & 300.00 & 12673 \\
Harnet & reachability & 11.87 & 0.20 & 300.00 & 1497 \\
Janetlense & reachability & 11.98 & 0.04 & 300.00 & 6937 \\
Janetlense & reachability & 11.98 & 0.19 & 300.00 & 1594 \\
Packetexchange & reachability & 11.99 & 0.04 & 300.00 & 8258 \\
Packetexchange & reachability & 11.99 & 0.19 & 300.00 & 1555 \\
Bandcon & reachability & 12.07 & 0.04 & 300.00 & 8213 \\
Bandcon & reachability & 12.07 & 0.27 & 300.00 & 1125 \\
Belnet2007 & reachability & 12.24 & 0.04 & 300.00 & 6938 \\
Belnet2007 & reachability & 12.24 & 0.20 & 300.00 & 1519 \\
Belnet2008 & reachability & 12.24 & 0.04 & 300.00 & 6988 \\
Belnet2008 & reachability & 12.24 & 0.20 & 300.00 & 1531 \\
Belnet2009 & reachability & 12.25 & 0.04 & 300.00 & 7423 \\
Belnet2009 & reachability & 12.25 & 0.19 & 300.00 & 1593 \\
Garr200109 & reachability & 12.76 & 0.02 & 300.00 & 12781 \\
Garr200109 & reachability & 12.76 & 0.20 & 300.00 & 1527 \\
Garr200404 & reachability & 12.76 & 0.02 & 300.00 & 12443 \\
Garr200404 & reachability & 12.76 & 0.19 & 300.00 & 1551 \\
KentmanApr2007 & reachability & 12.79 & 0.04 & 300.00 & 7847 \\
KentmanApr2007 & reachability & 12.79 & 0.23 & 300.00 & 1322 \\
Azrena & reachability & 12.82 & 0.03 & 300.00 & 9173 \\
Azrena & reachability & 12.82 & 0.22 & 300.00 & 1393 \\
HiberniaUs & reachability & 13.09 & 0.03 & 300.00 & 10690 \\
HiberniaUs & reachability & 13.09 & 0.23 & 300.00 & 1298 \\
Belnet2010 & reachability & 13.28 & 0.05 & 300.00 & 6044 \\
Belnet2010 & reachability & 13.28 & 0.22 & 300.00 & 1371 \\
Istar & reachability & 13.72 & 0.04 & 300.00 & 7684 \\
Istar & reachability & 13.72 & 0.24 & 300.00 & 1226 \\
Cesnet2001 & reachability & 13.73 & 0.03 & 300.00 & 11061 \\
Cesnet2001 & reachability & 13.73 & 0.22 & 300.00 & 1375 \\
York & reachability & 13.78 & 0.04 & 300.00 & 6964 \\
York & reachability & 13.78 & 0.29 & 300.00 & 1024 \\
Garr199904 & reachability & 13.85 & 0.03 & 300.00 & 9479 \\
Garr199904 & reachability & 13.85 & 0.22 & 300.00 & 1379 \\
Garr199905 & reachability & 13.85 & 0.03 & 300.00 & 8973 \\
Garr199905 & reachability & 13.85 & 0.21 & 300.00 & 1406 \\
Fccn & reachability & 13.99 & 0.03 & 300.00 & 10280 \\
Fccn & reachability & 13.99 & 0.26 & 300.00 & 1152 \\
Aconet & reachability & 14.24 & 0.10 & 300.00 & 3157 \\
Aconet & reachability & 14.24 & 0.30 & 300.00 & 991 \\
Abvt & reachability & 14.24 & 0.10 & 300.00 & 2860 \\
Abvt & reachability & 14.24 & 0.33 & 300.00 & 920 \\
VisionNet & reachability & 14.78 & 0.04 & 300.00 & 8176 \\
VisionNet & reachability & 14.78 & 0.33 & 300.00 & 922 \\
Renater1999 & reachability & 14.78 & 0.04 & 300.00 & 6914 \\
Renater1999 & reachability & 14.78 & 0.27 & 300.00 & 1113 \\
Uran & reachability & 14.85 & 0.03 & 300.00 & 9934 \\
Uran & reachability & 14.85 & 0.28 & 300.00 & 1090 \\
Psinet & reachability & 14.91 & 0.05 & 300.00 & 6153 \\
Psinet & reachability & 14.91 & 0.31 & 300.00 & 968 \\
Garr200112 & reachability & 14.97 & 0.03 & 300.00 & 10903 \\
Garr200112 & reachability & 14.97 & 0.24 & 300.00 & 1245 \\
Belnet2003 & reachability & 15.04 & 0.05 & 300.00 & 5907 \\
Belnet2003 & reachability & 15.04 & 0.22 & 300.00 & 1355 \\
Belnet2004 & reachability & 15.04 & 0.05 & 300.00 & 6007 \\
Belnet2004 & reachability & 15.04 & 0.23 & 300.00 & 1289 \\
Renater2001 & reachability & 15.04 & 0.05 & 300.00 & 6526 \\
Renater2001 & reachability & 15.04 & 0.25 & 300.00 & 1207 \\
Belnet2005 & reachability & 15.11 & 0.05 & 300.00 & 5696 \\
Belnet2005 & reachability & 15.11 & 0.25 & 300.00 & 1190 \\
Belnet2006 & reachability & 15.11 & 0.05 & 300.00 & 6088 \\
Belnet2006 & reachability & 15.11 & 0.25 & 300.00 & 1202 \\
Xeex & reachability & 15.50 & 0.04 & 300.00 & 6788 \\
Xeex & reachability & 15.50 & 0.25 & 300.00 & 1211 \\
HurricaneElectric & reachability & 15.69 & 0.03 & 300.00 & 9375 \\
HurricaneElectric & reachability & 15.69 & 0.24 & 300.00 & 1236 \\
BtEurope & reachability & 15.71 & 0.05 & 300.00 & 5991 \\
BtEurope & reachability & 15.71 & 0.27 & 300.00 & 1128 \\
Amres & reachability & 15.95 & 0.06 & 300.00 & 4990 \\
Amres & reachability & 15.95 & 0.40 & 300.00 & 746 \\
Vinaren & reachability & 16.07 & 0.04 & 300.00 & 7723 \\
Vinaren & reachability & 16.07 & 0.27 & 300.00 & 1107 \\
Arpanet19723 & reachability & 16.21 & 0.07 & 300.00 & 4255 \\
Arpanet19723 & reachability & 16.21 & 0.33 & 300.00 & 912 \\
UniC & reachability & 16.27 & 0.03 & 300.00 & 8879 \\
UniC & reachability & 16.27 & 0.32 & 300.00 & 951 \\
Karen & reachability & 16.33 & 0.04 & 300.00 & 6759 \\
Karen & reachability & 16.33 & 0.31 & 300.00 & 969 \\
Agis & reachability & 16.34 & 0.08 & 300.00 & 3937 \\
Agis & reachability & 16.34 & 0.34 & 300.00 & 875 \\
KentmanFeb2008 & reachability & 17.37 & 0.05 & 300.00 & 5913 \\
KentmanFeb2008 & reachability & 17.37 & 0.30 & 300.00 & 987 \\
Funet & reachability & 17.55 & 0.04 & 300.00 & 7503 \\
Funet & reachability & 17.55 & 0.36 & 300.00 & 823 \\
AttMpls & reachability & 18.10 & 0.05 & 300.00 & 5781 \\
AttMpls & reachability & 18.10 & 0.28 & 300.00 & 1085 \\
Bbnplanet & reachability & 18.55 & 0.05 & 300.00 & 6151 \\
Bbnplanet & reachability & 18.55 & 0.37 & 300.00 & 804 \\
Garr200212 & reachability & 18.62 & 0.04 & 300.00 & 8443 \\
Garr200212 & reachability & 18.62 & 0.34 & 300.00 & 895 \\
KentmanAug2005 & reachability & 18.67 & 0.06 & 300.00 & 5125 \\
KentmanAug2005 & reachability & 18.67 & 0.40 & 300.00 & 751 \\
Sunet & reachability & 18.73 & 0.04 & 300.00 & 7236 \\
Sunet & reachability & 18.73 & 0.37 & 300.00 & 812 \\
Integra & reachability & 19.07 & 0.04 & 300.00 & 7486 \\
Integra & reachability & 19.07 & 0.33 & 300.00 & 909 \\
Geant2001 & reachability & 19.19 & 0.04 & 300.00 & 7857 \\
Geant2001 & reachability & 19.19 & 0.32 & 300.00 & 950 \\
Gambia & reachability & 19.80 & 0.04 & 300.00 & 7151 \\
Gambia & reachability & 19.80 & 0.40 & 300.00 & 747 \\
Darkstrand & reachability & 19.98 & 0.07 & 300.00 & 4396 \\
Darkstrand & reachability & 19.98 & 0.42 & 300.00 & 717 \\
Shentel & reachability & 20.25 & 0.04 & 300.00 & 6725 \\
Shentel & reachability & 20.25 & 0.45 & 300.00 & 670 \\
Arpanet19728 & reachability & 21.33 & 0.07 & 300.00 & 4560 \\
Arpanet19728 & reachability & 21.33 & 0.50 & 300.00 & 604 \\
Biznet & reachability & 21.40 & 0.05 & 300.00 & 5705 \\
Biznet & reachability & 21.40 & 0.51 & 300.00 & 593 \\
Cesnet200304 & reachability & 21.40 & 0.05 & 300.00 & 6618 \\
Cesnet200304 & reachability & 21.40 & 0.39 & 300.00 & 762 \\
Janetbackbone & reachability & 22.19 & 0.07 & 300.00 & 4073 \\
Janetbackbone & reachability & 22.19 & 0.40 & 300.00 & 745 \\
Arn & reachability & 22.47 & 0.11 & 300.00 & 2673 \\
Arn & reachability & 22.47 & 0.60 & 300.00 & 504 \\
Cynet & reachability & 22.49 & 0.07 & 300.00 & 4156 \\
Cynet & reachability & 22.49 & 0.47 & 300.00 & 636 \\
GtsHungary & reachability & 22.62 & 0.05 & 300.00 & 6003 \\
GtsHungary & reachability & 22.62 & 0.55 & 300.00 & 549 \\
Ernet & reachability & 22.66 & 0.04 & 300.00 & 6774 \\
Ernet & reachability & 22.66 & 0.43 & 300.00 & 690 \\
WideJpn & reachability & 22.72 & 0.06 & 300.00 & 5378 \\
WideJpn & reachability & 22.72 & 0.42 & 300.00 & 716 \\
Renater2004 & reachability & 22.94 & 0.08 & 300.00 & 3736 \\
Renater2004 & reachability & 22.94 & 0.45 & 300.00 & 670 \\
Rnp & reachability & 24.15 & 0.06 & 300.00 & 5237 \\
Rnp & reachability & 24.15 & 0.56 & 300.00 & 536 \\
Iinet & reachability & 24.24 & 0.05 & 300.00 & 6191 \\
Iinet & reachability & 24.24 & 0.47 & 300.00 & 645 \\
Digex & reachability & 24.42 & 0.07 & 300.00 & 4442 \\
Digex & reachability & 24.42 & 0.57 & 300.00 & 530 \\
GtsCzechRepublic & reachability & 25.50 & 0.05 & 300.00 & 5513 \\
GtsCzechRepublic & reachability & 25.50 & 0.61 & 300.00 & 492 \\
DeutscheTelekom & reachability & 25.99 & 0.93 & 300.00 & 323 \\
Canerie & reachability & 26.02 & 0.05 & 300.00 & 5608 \\
Canerie & reachability & 26.02 & 0.55 & 300.00 & 548 \\
GtsPoland & reachability & 27.22 & 0.06 & 300.00 & 4997 \\
GtsPoland & reachability & 27.22 & 0.65 & 300.00 & 462 \\
CrlNetworkServices & reachability & 27.28 & 0.09 & 300.00 & 3349 \\
CrlNetworkServices & reachability & 27.28 & 0.59 & 300.00 & 512 \\
IowaStatewideFiberMap & reachability & 27.48 & 0.06 & 300.00 & 5046 \\
IowaStatewideFiberMap & reachability & 27.48 & 0.63 & 300.00 & 475 \\
Renater2006 & reachability & 27.62 & 0.08 & 300.00 & 3629 \\
Renater2006 & reachability & 27.62 & 0.55 & 300.00 & 546 \\
Renater2008 & reachability & 27.62 & 0.06 & 300.00 & 4812 \\
Renater2008 & reachability & 27.62 & 0.57 & 300.00 & 531 \\
Bics & reachability & 27.94 & 0.06 & 300.00 & 4688 \\
Bics & reachability & 27.94 & 0.57 & 300.00 & 526 \\
Arnes & reachability & 29.37 & 0.14 & 300.00 & 2168 \\
Arnes & reachability & 29.37 & 0.78 & 300.00 & 384 \\
Xspedius & reachability & 29.51 & 0.08 & 300.00 & 3604 \\
Xspedius & reachability & 29.51 & 0.59 & 300.00 & 511 \\
Geant2009 & reachability & 29.69 & 0.07 & 300.00 & 4252 \\
Geant2009 & reachability & 29.69 & 0.58 & 300.00 & 519 \\
Zamren & reachability & 30.12 & 0.07 & 300.00 & 4142 \\
Zamren & reachability & 30.12 & 0.83 & 300.00 & 359 \\
GtsSlovakia & reachability & 30.33 & 0.06 & 300.00 & 4845 \\
GtsSlovakia & reachability & 30.33 & 0.73 & 300.00 & 412 \\
NetworkUsa & reachability & 30.39 & 0.11 & 300.00 & 2824 \\
NetworkUsa & reachability & 30.39 & 0.77 & 300.00 & 391 \\
Cwix & reachability & 32.10 & 0.10 & 300.00 & 2933 \\
Cwix & reachability & 32.10 & 0.77 & 300.00 & 392 \\
PionierL1 & reachability & 32.12 & 0.10 & 300.00 & 2893 \\
PionierL1 & reachability & 32.12 & 0.75 & 300.00 & 397 \\
Niif & reachability & 32.13 & 0.11 & 300.00 & 2809 \\
Niif & reachability & 32.13 & 0.69 & 300.00 & 433 \\
Reuna & reachability & 33.43 & 0.16 & 300.00 & 1833 \\
Reuna & reachability & 33.43 & 0.86 & 300.00 & 347 \\
Bren & reachability & 33.55 & 0.08 & 300.00 & 3568 \\
Bren & reachability & 33.55 & 0.75 & 300.00 & 401 \\
Myren & reachability & 33.75 & 0.10 & 300.00 & 3003 \\
Myren & reachability & 33.75 & 0.69 & 300.00 & 432 \\
Evolink & reachability & 34.03 & 0.08 & 300.00 & 3756 \\
Evolink & reachability & 34.03 & 0.88 & 300.00 & 341 \\
Grnet & reachability & 34.16 & 0.07 & 300.00 & 4325 \\
Grnet & reachability & 34.16 & 0.76 & 300.00 & 395 \\
BtNorthAmerica & reachability & 34.41 & 0.09 & 300.00 & 3430 \\
BtNorthAmerica & reachability & 34.41 & 0.67 & 300.00 & 450 \\
Geant2010 & reachability & 34.85 & 0.08 & 300.00 & 3759 \\
Geant2010 & reachability & 34.85 & 0.72 & 300.00 & 416 \\
KentmanJan2011 & reachability & 35.30 & 0.10 & 300.00 & 2967 \\
KentmanJan2011 & reachability & 35.30 & 0.82 & 300.00 & 366 \\
Iij & reachability & 35.46 & 0.08 & 300.00 & 3673 \\
Iij & reachability & 35.46 & 0.80 & 300.00 & 377 \\
PionierL3 & reachability & 36.14 & 0.12 & 300.00 & 2458 \\
PionierL3 & reachability & 36.14 & 0.85 & 300.00 & 352 \\
Cesnet200511 & reachability & 37.35 & 0.08 & 300.00 & 3776 \\
Cesnet200511 & reachability & 37.35 & 0.85 & 300.00 & 354 \\
Cesnet200603 & reachability & 37.35 & 0.09 & 300.00 & 3509 \\
Cesnet200603 & reachability & 37.35 & 0.87 & 300.00 & 344 \\
Intranetwork & reachability & 37.93 & 0.10 & 300.00 & 3033 \\
Intranetwork & reachability & 37.93 & 1.12 & 300.00 & 269 \\
Ntt & reachability & 38.25 & 0.17 & 300.00 & 1745 \\
Ntt & reachability & 38.25 & 1.13 & 300.00 & 265 \\
Geant2012 & reachability & 40.20 & 0.09 & 300.00 & 3392 \\
Geant2012 & reachability & 40.20 & 0.90 & 300.00 & 332 \\
Cernet & reachability & 41.94 & 0.13 & 300.00 & 2346 \\
Cernet & reachability & 41.94 & 0.97 & 300.00 & 309 \\
LambdaNet & reachability & 42.90 & 0.15 & 300.00 & 1964 \\
LambdaNet & reachability & 42.90 & 1.38 & 300.00 & 217 \\
Roedunet & reachability & 43.19 & 0.09 & 300.00 & 3176 \\
Roedunet & reachability & 43.19 & 1.08 & 300.00 & 279 \\
SwitchL3 & reachability & 44.00 & 0.10 & 300.00 & 3058 \\
SwitchL3 & reachability & 44.00 & 0.95 & 300.00 & 315 \\
Chinanet & reachability & 44.31 & 0.16 & 300.00 & 1888 \\
Chinanet & reachability & 44.31 & 1.03 & 300.00 & 293 \\
Litnet & reachability & 44.62 & 0.12 & 300.00 & 2449 \\
Litnet & reachability & 44.62 & 0.99 & 300.00 & 303 \\
Sanet & reachability & 44.73 & 0.10 & 300.00 & 3014 \\
Sanet & reachability & 44.73 & 1.35 & 300.00 & 222 \\
Renater2010 & reachability & 45.45 & 0.10 & 300.00 & 2976 \\
Renater2010 & reachability & 45.45 & 1.15 & 300.00 & 261 \\
Carnet & reachability & 46.58 & 0.10 & 300.00 & 2919 \\
Carnet & reachability & 46.58 & 1.33 & 300.00 & 225 \\
Cesnet200706 & reachability & 47.08 & 0.10 & 300.00 & 3028 \\
Cesnet200706 & reachability & 47.08 & 1.15 & 300.00 & 261 \\
BtLatinAmerica & reachability & 49.04 & 0.09 & 300.00 & 3182 \\
BtLatinAmerica & reachability & 49.04 & 1.99 & 300.00 & 150 \\
Palmetto & reachability & 50.29 & 0.17 & 300.00 & 1764 \\
Palmetto & reachability & 50.29 & 1.33 & 300.00 & 226 \\
Ntelos & reachability & 53.81 & 0.18 & 300.00 & 1687 \\
Ntelos & reachability & 53.81 & 1.84 & 300.00 & 163 \\
RoedunetFibre & reachability & 55.33 & 0.13 & 300.00 & 2359 \\
RoedunetFibre & reachability & 55.33 & 1.60 & 300.00 & 188 \\
Bellcanada & reachability & 56.19 & 0.17 & 300.00 & 1788 \\
Bellcanada & reachability & 56.19 & 1.69 & 300.00 & 177 \\
Uunet & reachability & 59.60 & 0.18 & 300.00 & 1661 \\
Uunet & reachability & 59.60 & 1.43 & 300.00 & 209 \\
Surfnet & reachability & 61.07 & 0.14 & 300.00 & 2165 \\
Surfnet & reachability & 61.07 & 1.70 & 300.00 & 176 \\
Cudi & reachability & 61.98 & 0.18 & 300.00 & 1663 \\
Cudi & reachability & 61.98 & 1.63 & 300.00 & 184 \\
Iris & reachability & 62.73 & 0.19 & 300.00 & 1580 \\
Iris & reachability & 62.73 & 1.90 & 300.00 & 158 \\
Bellsouth & reachability & 62.95 & 0.22 & 300.00 & 1368 \\
Bellsouth & reachability & 62.95 & 1.98 & 300.00 & 152 \\
Cesnet201006 & reachability & 64.99 & 0.23 & 300.00 & 1284 \\
Cesnet201006 & reachability & 64.99 & 1.85 & 300.00 & 162 \\
BeyondTheNetwork & reachability & 67.41 & 0.14 & 300.00 & 2160 \\
BeyondTheNetwork & reachability & 67.41 & 1.83 & 300.00 & 164 \\
Tinet & reachability & 69.00 & 0.16 & 300.00 & 1887 \\
Tinet & reachability & 69.00 & 1.83 & 300.00 & 164 \\
Garr200912 & reachability & 70.01 & 0.15 & 300.00 & 1965 \\
Garr200912 & reachability & 70.01 & 1.91 & 300.00 & 157 \\
Garr201001 & reachability & 70.01 & 0.14 & 300.00 & 2077 \\
Garr201001 & reachability & 70.01 & 1.84 & 300.00 & 163 \\
Garr200908 & reachability & 70.01 & 0.14 & 300.00 & 2092 \\
Garr200908 & reachability & 70.01 & 1.86 & 300.00 & 161 \\
Garr201003 & reachability & 70.21 & 0.15 & 300.00 & 2066 \\
Garr201003 & reachability & 70.21 & 1.85 & 300.00 & 162 \\
Garr201004 & reachability & 70.21 & 0.15 & 300.00 & 2040 \\
Garr201004 & reachability & 70.21 & 1.88 & 300.00 & 159 \\
Garr200902 & reachability & 70.22 & 0.14 & 300.00 & 2074 \\
Garr200902 & reachability & 70.22 & 1.81 & 300.00 & 166 \\
Garr200909 & reachability & 72.50 & 0.17 & 300.00 & 1771 \\
Garr200909 & reachability & 72.50 & 2.02 & 300.00 & 148 \\
Garr201005 & reachability & 72.71 & 0.16 & 300.00 & 1929 \\
Garr201005 & reachability & 72.71 & 1.96 & 300.00 & 153 \\
Garr201007 & reachability & 72.84 & 0.15 & 300.00 & 2037 \\
Garr201007 & reachability & 72.84 & 1.89 & 300.00 & 158 \\
Garr201008 & reachability & 72.84 & 0.15 & 300.00 & 2016 \\
Garr201008 & reachability & 72.84 & 1.89 & 300.00 & 158 \\
HiberniaGlobal & reachability & 73.28 & 0.16 & 300.00 & 1903 \\
HiberniaGlobal & reachability & 73.28 & 2.53 & 300.00 & 119 \\
Garr201010 & reachability & 75.37 & 0.15 & 300.00 & 1986 \\
Garr201010 & reachability & 75.37 & 2.01 & 300.00 & 149 \\
Garr201012 & reachability & 75.37 & 0.15 & 300.00 & 1973 \\
Garr201012 & reachability & 75.37 & 2.01 & 300.00 & 149 \\
Garr201101 & reachability & 75.44 & 0.16 & 300.00 & 1918 \\
Garr201101 & reachability & 75.44 & 2.07 & 300.00 & 145 \\
Garr201102 & reachability & 78.02 & 0.16 & 300.00 & 1873 \\
Garr201102 & reachability & 78.02 & 2.19 & 300.00 & 137 \\
Garr201103 & reachability & 80.85 & 0.17 & 300.00 & 1776 \\
Garr201103 & reachability & 80.85 & 2.46 & 300.00 & 122 \\
Dfn & reachability & 81.30 & 0.23 & 300.00 & 1309 \\
Dfn & reachability & 81.30 & 2.65 & 300.00 & 113 \\
Garr201104 & reachability & 83.59 & 0.20 & 300.00 & 1474 \\
Garr201104 & reachability & 83.59 & 2.37 & 300.00 & 127 \\
Garr201105 & reachability & 83.69 & 0.18 & 300.00 & 1676 \\
Garr201105 & reachability & 83.69 & 2.36 & 300.00 & 127 \\
Garr201107 & reachability & 83.76 & 0.17 & 300.00 & 1721 \\
Garr201107 & reachability & 83.76 & 2.32 & 300.00 & 129 \\
Garr201108 & reachability & 83.76 & 0.17 & 300.00 & 1746 \\
Garr201108 & reachability & 83.76 & 2.36 & 300.00 & 127 \\
Garr201109 & reachability & 83.82 & 0.17 & 300.00 & 1760 \\
Garr201109 & reachability & 83.82 & 2.47 & 300.00 & 121 \\
Garr201110 & reachability & 83.91 & 0.17 & 300.00 & 1725 \\
Garr201110 & reachability & 83.91 & 2.51 & 300.00 & 120 \\
Garr201111 & reachability & 86.55 & 0.18 & 300.00 & 1626 \\
Garr201111 & reachability & 86.55 & 2.62 & 300.00 & 115 \\
UsSignal & reachability & 88.70 & 0.25 & 300.00 & 1218 \\
UsSignal & reachability & 88.70 & 3.29 & 300.00 & 91 \\
Garr201112 & reachability & 89.38 & 0.19 & 300.00 & 1600 \\
Garr201112 & reachability & 89.38 & 2.70 & 300.00 & 111 \\
Garr201201 & reachability & 89.38 & 0.19 & 300.00 & 1581 \\
Garr201201 & reachability & 89.38 & 2.53 & 300.00 & 119 \\
Forthnet & reachability & 90.29 & 0.18 & 300.00 & 1712 \\
Forthnet & reachability & 90.29 & 3.18 & 300.00 & 94 \\
AsnetAm & reachability & 99.88 & 0.26 & 300.00 & 1151 \\
AsnetAm & reachability & 99.88 & 3.60 & 300.00 & 83 \\
Internode & reachability & 102.65 & 0.19 & 300.00 & 1553 \\
Internode & reachability & 102.65 & 3.06 & 300.00 & 98 \\
Missouri & reachability & 105.94 & 0.34 & 300.00 & 883 \\
Missouri & reachability & 105.94 & 3.86 & 300.00 & 78 \\
Globenet & reachability & 107.92 & 0.23 & 300.00 & 1313 \\
Globenet & reachability & 107.92 & 3.70 & 300.00 & 81 \\
Esnet & reachability & 109.59 & 0.22 & 300.00 & 1349 \\
Esnet & reachability & 109.59 & 3.90 & 300.00 & 77 \\
Latnet & reachability & 111.48 & 0.39 & 300.00 & 776 \\
Latnet & reachability & 111.48 & 5.04 & 300.00 & 60 \\
Uninett2011 & reachability & 112.95 & 0.25 & 300.00 & 1193 \\
Uninett2011 & reachability & 112.95 & 3.52 & 300.00 & 85 \\
Columbus & reachability & 115.19 & 0.28 & 300.00 & 1076 \\
Columbus & reachability & 115.19 & 4.64 & 300.00 & 65 \\
Telcove & reachability & 117.45 & 0.23 & 300.00 & 1315 \\
Telcove & reachability & 117.45 & 4.43 & 300.00 & 68 \\
Tw & reachability & 120.57 & 0.28 & 300.00 & 1090 \\
Tw & reachability & 120.57 & 4.23 & 300.00 & 71 \\
Intellifiber & reachability & 125.49 & 0.27 & 300.00 & 1104 \\
Intellifiber & reachability & 125.49 & 4.82 & 300.00 & 62 \\
Syringa & reachability & 127.24 & 0.35 & 300.00 & 864 \\
Syringa & reachability & 127.24 & 7.58 & 300.00 & 40 \\
Sinet & reachability & 127.41 & 0.25 & 300.00 & 1183 \\
Sinet & reachability & 127.41 & 4.39 & 300.00 & 68 \\
Switch & reachability & 128.43 & 0.28 & 300.00 & 1073 \\
Switch & reachability & 128.43 & 5.02 & 300.00 & 60 \\
Uninett2010 & reachability & 129.01 & 0.27 & 300.00 & 1105 \\
Uninett2010 & reachability & 129.01 & 4.17 & 300.00 & 72 \\
Ulaknet & reachability & 155.63 & 0.43 & 300.00 & 690 \\
Ulaknet & reachability & 155.63 & 12.73 & 300.00 & 24 \\
Oteglobe & reachability & 161.66 & 8.56 & 300.00 & 35 \\
RedBestel & reachability & 164.04 & 0.57 & 300.00 & 525 \\
RedBestel & reachability & 164.04 & 9.47 & 300.00 & 32 \\
VtlWavenet2008 & reachability & 178.69 & 0.66 & 300.00 & 457 \\
VtlWavenet2008 & reachability & 178.69 & 11.72 & 300.00 & 26 \\
VtlWavenet2011 & reachability & 194.90 & 0.71 & 300.00 & 421 \\
VtlWavenet2011 & reachability & 194.90 & 13.04 & 300.00 & 23 \\
Interoute & reachability & 280.54 & 0.65 & 300.00 & 464 \\
Interoute & reachability & 280.54 & 14.66 & 300.00 & 20 \\
Deltacom & reachability & 297.44 & 1.10 & 300.00 & 273 \\
Deltacom & reachability & 297.44 & 17.03 & 300.00 & 18 \\
Ion & reachability & 360.16 & 0.98 & 300.00 & 305 \\
Ion & reachability & 360.16 & 24.15 & 300.00 & 12 \\
Pern & reachability & 370.66 & 1.11 & 300.00 & 270 \\
Pern & reachability & 370.66 & 21.70 & 300.00 & 14 \\
DialtelecomCz & reachability & 443.13 & 1.23 & 300.00 & 244 \\
DialtelecomCz & reachability & 443.13 & 62.13 & 300.00 & 5 \\
TataNld & reachability & 485.91 & 1.28 & 300.00 & 234 \\
TataNld & reachability & 485.91 & 32.92 & 300.00 & 9 \\
GtsCe & reachability & 512.65 & 1.47 & 300.00 & 203 \\
GtsCe & reachability & 512.65 & 34.82 & 300.00 & 9 \\
Colt & reachability & 540.17 & 1.66 & 300.00 & 181 \\
Colt & reachability & 540.17 & 37.43 & 300.00 & 8 \\
UsCarrier & reachability & 575.29 & 1.71 & 300.00 & 176 \\
UsCarrier & reachability & 575.29 & 45.41 & 300.00 & 7 \\
Cogentco & reachability & 894.78 & 2.61 & 300.00 & 115 \\
Cogentco & reachability & 894.78 & 77.62 & 300.00 & 4 \\
\bottomrule
\end{tabular}


==> plots/Full_reachability_comparison_table_old.tex <==
\begin{tabular}{llrrrr}
\toprule
Name & Type & Size & KATch (s) & Frenetic (s) & Speedup \\
\midrule
Arpanet196912 & reachability & 71 & 0.01 & 0.30 & 50 \\
Arpanet196912 & reachability & 71 & 0.01 & 0.30 & 45 \\
Renam & reachability & 92 & 0.00 & 0.53 & 140 \\
Renam & reachability & 92 & 0.01 & 0.53 & 84 \\
Mren & reachability & 123 & 0.00 & 1.11 & 231 \\
Mren & reachability & 123 & 0.01 & 1.11 & 122 \\
Telecomserbia & reachability & 129 & 0.00 & 0.97 & 245 \\
Telecomserbia & reachability & 129 & 0.01 & 0.97 & 102 \\
Epoch & reachability & 135 & 0.00 & 0.91 & 220 \\
Epoch & reachability & 135 & 0.01 & 0.91 & 98 \\
Layer42 & reachability & 135 & 0.01 & 1.11 & 204 \\
Layer42 & reachability & 135 & 0.01 & 1.11 & 124 \\
Napnet & reachability & 135 & 0.01 & 1.06 & 196 \\
Napnet & reachability & 135 & 0.01 & 1.06 & 118 \\
Basnet & reachability & 158 & 0.01 & 2.01 & 317 \\
Basnet & reachability & 158 & 0.02 & 2.01 & 118 \\
Nordu1989 & reachability & 158 & 0.01 & 1.93 & 326 \\
Nordu1989 & reachability & 158 & 0.01 & 1.93 & 146 \\
Dataxchange & reachability & 159 & 0.01 & 1.19 & 190 \\
Dataxchange & reachability & 159 & 0.01 & 1.19 & 130 \\
Sanren & reachability & 164 & 0.00 & 1.69 & 366 \\
Sanren & reachability & 164 & 0.01 & 1.69 & 125 \\
Padi & reachability & 166 & 0.01 & 7.57 & 1303 \\
Padi & reachability & 166 & 0.04 & 7.57 & 181 \\
Getnet & reachability & 170 & 0.00 & 1.82 & 390 \\
Getnet & reachability & 170 & 0.01 & 1.82 & 133 \\
Netrail & reachability & 182 & 0.01 & 2.06 & 293 \\
Netrail & reachability & 182 & 0.01 & 2.06 & 166 \\
Gblnet & reachability & 197 & 0.01 & 3.40 & 609 \\
Gblnet & reachability & 197 & 0.02 & 3.40 & 180 \\
Heanet & reachability & 200 & 0.01 & 2.20 & 408 \\
Heanet & reachability & 200 & 0.01 & 2.20 & 152 \\
HiberniaIreland & reachability & 203 & 0.01 & 3.35 & 582 \\
HiberniaIreland & reachability & 203 & 0.02 & 3.35 & 178 \\
Arpanet19706 & reachability & 252 & 0.01 & 5.17 & 385 \\
Arpanet19706 & reachability & 252 & 0.03 & 5.17 & 157 \\
Nordu2005 & reachability & 252 & 0.01 & 6.13 & 659 \\
Nordu2005 & reachability & 252 & 0.03 & 6.13 & 199 \\
Nsfcnet & reachability & 253 & 0.01 & 7.03 & 737 \\
Nsfcnet & reachability & 253 & 0.03 & 7.03 & 221 \\
Ai3 & reachability & 287 & 0.02 & 9.33 & 522 \\
Ai3 & reachability & 287 & 0.04 & 9.33 & 212 \\
Cesnet1993 & reachability & 287 & 0.01 & 9.44 & 1184 \\
Cesnet1993 & reachability & 287 & 0.03 & 9.44 & 315 \\
JanetExternal & reachability & 307 & 0.05 & 14.68 & 283 \\
Gridnet & reachability & 312 & 0.01 & 6.34 & 783 \\
Gridnet & reachability & 312 & 0.02 & 6.34 & 279 \\
Itnet & reachability & 338 & 0.01 & 18.80 & 1619 \\
Itnet & reachability & 338 & 0.04 & 18.80 & 459 \\
Singaren & reachability & 338 & 0.01 & 18.59 & 1954 \\
Singaren & reachability & 338 & 0.04 & 18.59 & 471 \\
Abilene & reachability & 362 & 0.05 & 12.78 & 273 \\
Abilene & reachability & 362 & 0.07 & 12.78 & 174 \\
Sprint & reachability & 386 & 0.01 & 14.61 & 1473 \\
Sprint & reachability & 386 & 0.04 & 14.61 & 396 \\
Globalcenter & reachability & 408 & 0.01 & 6.92 & 842 \\
Globalcenter & reachability & 408 & 0.02 & 6.92 & 327 \\
TLex & reachability & 423 & 0.01 & 28.18 & 2508 \\
TLex & reachability & 423 & 0.05 & 28.18 & 587 \\
Cesnet1997 & reachability & 452 & 0.01 & 35.05 & 3150 \\
Cesnet1997 & reachability & 452 & 0.06 & 35.05 & 586 \\
Cesnet1999 & reachability & 452 & 0.01 & 38.99 & 3479 \\
Cesnet1999 & reachability & 452 & 0.06 & 38.99 & 656 \\
Kreonet & reachability & 452 & 0.02 & 41.72 & 2592 \\
Kreonet & reachability & 452 & 0.06 & 41.72 & 732 \\
HiberniaCanada & reachability & 464 & 0.01 & 30.65 & 2649 \\
HiberniaCanada & reachability & 464 & 0.07 & 30.65 & 469 \\
Nsfnet & reachability & 470 & 0.02 & 31.40 & 1886 \\
Nsfnet & reachability & 470 & 0.05 & 31.40 & 580 \\
Eenet & reachability & 476 & 0.01 & 45.15 & 3818 \\
Eenet & reachability & 476 & 0.06 & 45.15 & 733 \\
Navigata & reachability & 482 & 0.02 & 37.02 & 2196 \\
Navigata & reachability & 482 & 0.06 & 37.02 & 668 \\
Nordu1997 & reachability & 515 & 0.02 & 70.83 & 4007 \\
Nordu1997 & reachability & 515 & 0.07 & 70.83 & 1061 \\
Ilan & reachability & 527 & 0.01 & 55.71 & 4718 \\
Ilan & reachability & 527 & 0.07 & 55.71 & 796 \\
Uninet & reachability & 530 & 0.01 & 38.85 & 2898 \\
Uninet & reachability & 530 & 0.06 & 38.85 & 668 \\
Compuserve & reachability & 539 & 0.02 & 62.47 & 2980 \\
Compuserve & reachability & 539 & 0.07 & 62.47 & 951 \\
Eunetworks & reachability & 552 & 0.02 & 51.63 & 3409 \\
Eunetworks & reachability & 552 & 0.09 & 51.63 & 581 \\
HiberniaUk & reachability & 588 & 0.01 & 66.54 & 4491 \\
HiberniaUk & reachability & 588 & 0.09 & 66.54 & 719 \\
Spiralight & reachability & 594 & 0.02 & 69.02 & 4306 \\
Spiralight & reachability & 594 & 0.09 & 69.02 & 798 \\
Claranet & reachability & 606 & 0.02 & 82.76 & 3743 \\
Claranet & reachability & 606 & 0.08 & 82.76 & 1068 \\
Nordu2010 & reachability & 627 & 0.13 & 133.85 & 1022 \\
Grena & reachability & 653 & 0.01 & 95.49 & 6479 \\
Grena & reachability & 653 & 0.11 & 95.49 & 835 \\
KentmanJul2005 & reachability & 665 & 0.02 & 114.01 & 5184 \\
KentmanJul2005 & reachability & 665 & 0.09 & 114.01 & 1203 \\
Garr199901 & reachability & 671 & 0.02 & 129.77 & 8377 \\
Garr199901 & reachability & 671 & 0.09 & 129.77 & 1397 \\
Marwan & reachability & 671 & 0.02 & 102.47 & 4492 \\
Marwan & reachability & 671 & 0.10 & 102.47 & 1025 \\
Rhnet & reachability & 671 & 0.02 & 114.55 & 5803 \\
Rhnet & reachability & 671 & 0.11 & 114.55 & 1062 \\
Peer1 & reachability & 683 & 0.02 & 120.67 & 4904 \\
Peer1 & reachability & 683 & 0.10 & 120.67 & 1258 \\
HostwayInternational & reachability & 689 & 0.02 & 108.01 & 6589 \\
HostwayInternational & reachability & 689 & 0.10 & 108.01 & 1053 \\
Nextgen & reachability & 752 & 0.03 & 140.05 & 5310 \\
Nextgen & reachability & 752 & 0.12 & 140.05 & 1143 \\
Fatman & reachability & 758 & 0.02 & 180.77 & 9506 \\
Fatman & reachability & 758 & 0.12 & 180.77 & 1556 \\
Airtel & reachability & 785 & 0.05 & 195.12 & 4153 \\
Airtel & reachability & 785 & 0.13 & 195.12 & 1515 \\
Jgn2Plus & reachability & 807 & 0.03 & 227.89 & 8582 \\
Jgn2Plus & reachability & 807 & 0.15 & 227.89 & 1537 \\
Sago & reachability & 807 & 0.02 & 163.82 & 8256 \\
Sago & reachability & 807 & 0.17 & 163.82 & 961 \\
Goodnet & reachability & 818 & 0.02 & 211.21 & 10395 \\
Goodnet & reachability & 818 & 0.11 & 211.21 & 1983 \\
Arpanet19719 & reachability & 837 & 0.04 & 195.82 & 4792 \\
Arpanet19719 & reachability & 837 & 0.16 & 195.82 & 1199 \\
HiberniaNireland & reachability & 837 & 0.02 & 209.54 & 10412 \\
HiberniaNireland & reachability & 837 & 0.14 & 209.54 & 1538 \\
BsonetEurope & reachability & 849 & 0.03 & 248.80 & 8811 \\
BsonetEurope & reachability & 849 & 0.12 & 248.80 & 2053 \\
Ibm & reachability & 849 & 0.02 & 223.49 & 11199 \\
Ibm & reachability & 849 & 0.12 & 223.49 & 1820 \\
Ans & reachability & 855 & 0.04 & 228.42 & 6090 \\
Ans & reachability & 855 & 0.13 & 228.42 & 1821 \\
Pacificwave & reachability & 867 & 0.03 & 300.00 & 10552 \\
Pacificwave & reachability & 867 & 0.12 & 300.00 & 2532 \\
Savvis & reachability & 902 & 0.02 & 255.55 & 11464 \\
Savvis & reachability & 902 & 0.16 & 255.55 & 1565 \\
Restena & reachability & 908 & 0.02 & 300.00 & 14409 \\
Restena & reachability & 908 & 0.14 & 300.00 & 2107 \\
Aarnet & reachability & 926 & 0.51 & 271.58 & 532 \\
Aarnet & reachability & 926 & 0.84 & 271.58 & 323 \\
Noel & reachability & 932 & 0.03 & 300.00 & 9437 \\
Noel & reachability & 932 & 0.14 & 300.00 & 2183 \\
Easynet & reachability & 956 & 0.02 & 300.00 & 13589 \\
Easynet & reachability & 956 & 0.15 & 300.00 & 1975 \\
Rediris & reachability & 974 & 0.04 & 300.00 & 7904 \\
Rediris & reachability & 974 & 0.14 & 300.00 & 2172 \\
Twaren & reachability & 983 & 0.02 & 300.00 & 14296 \\
Twaren & reachability & 983 & 0.15 & 300.00 & 1961 \\
Oxford & reachability & 1019 & 0.03 & 300.00 & 8799 \\
Oxford & reachability & 1019 & 0.17 & 300.00 & 1771 \\
Highwinds & reachability & 1023 & 0.02 & 300.00 & 12038 \\
Highwinds & reachability & 1023 & 0.14 & 300.00 & 2174 \\
Marnet & reachability & 1025 & 0.06 & 300.00 & 5150 \\
Marnet & reachability & 1025 & 0.17 & 300.00 & 1757 \\
EliBackbone & reachability & 1043 & 0.02 & 300.00 & 12050 \\
EliBackbone & reachability & 1043 & 0.16 & 300.00 & 1864 \\
BtAsiaPac & reachability & 1049 & 0.04 & 300.00 & 7630 \\
BtAsiaPac & reachability & 1049 & 0.16 & 300.00 & 1887 \\
Quest & reachability & 1049 & 0.04 & 300.00 & 7890 \\
Quest & reachability & 1049 & 0.16 & 300.00 & 1927 \\
Internetmci & reachability & 1052 & 0.03 & 300.00 & 11357 \\
Internetmci & reachability & 1052 & 0.14 & 300.00 & 2101 \\
Atmnet & reachability & 1080 & 0.03 & 300.00 & 9509 \\
Atmnet & reachability & 1080 & 0.23 & 300.00 & 1322 \\
GtsRomania & reachability & 1092 & 0.02 & 300.00 & 12072 \\
GtsRomania & reachability & 1092 & 0.20 & 300.00 & 1517 \\
Harnet & reachability & 1098 & 0.02 & 300.00 & 12673 \\
Harnet & reachability & 1098 & 0.20 & 300.00 & 1497 \\
Janetlense & reachability & 1103 & 0.04 & 300.00 & 6937 \\
Janetlense & reachability & 1103 & 0.19 & 300.00 & 1594 \\
Packetexchange & reachability & 1110 & 0.04 & 300.00 & 8258 \\
Packetexchange & reachability & 1110 & 0.19 & 300.00 & 1555 \\
Bandcon & reachability & 1117 & 0.04 & 300.00 & 8213 \\
Bandcon & reachability & 1117 & 0.27 & 300.00 & 1125 \\
Belnet2007 & reachability & 1134 & 0.04 & 300.00 & 6938 \\
Belnet2007 & reachability & 1134 & 0.20 & 300.00 & 1519 \\
Belnet2008 & reachability & 1134 & 0.04 & 300.00 & 6988 \\
Belnet2008 & reachability & 1134 & 0.20 & 300.00 & 1531 \\
Belnet2009 & reachability & 1134 & 0.04 & 300.00 & 7423 \\
Belnet2009 & reachability & 1134 & 0.19 & 300.00 & 1593 \\
Garr200109 & reachability & 1181 & 0.02 & 300.00 & 12781 \\
Garr200109 & reachability & 1181 & 0.20 & 300.00 & 1527 \\
Garr200404 & reachability & 1181 & 0.02 & 300.00 & 12443 \\
Garr200404 & reachability & 1181 & 0.19 & 300.00 & 1551 \\
KentmanApr2007 & reachability & 1182 & 0.04 & 300.00 & 7847 \\
KentmanApr2007 & reachability & 1182 & 0.23 & 300.00 & 1322 \\
Azrena & reachability & 1187 & 0.03 & 300.00 & 9173 \\
Azrena & reachability & 1187 & 0.22 & 300.00 & 1393 \\
HiberniaUs & reachability & 1211 & 0.03 & 300.00 & 10690 \\
HiberniaUs & reachability & 1211 & 0.23 & 300.00 & 1298 \\
Belnet2010 & reachability & 1229 & 0.05 & 300.00 & 6044 \\
Belnet2010 & reachability & 1229 & 0.22 & 300.00 & 1371 \\
Cesnet2001 & reachability & 1268 & 0.03 & 300.00 & 11061 \\
Cesnet2001 & reachability & 1268 & 0.22 & 300.00 & 1375 \\
Istar & reachability & 1268 & 0.04 & 300.00 & 7684 \\
Istar & reachability & 1268 & 0.24 & 300.00 & 1226 \\
York & reachability & 1274 & 0.04 & 300.00 & 6964 \\
York & reachability & 1274 & 0.29 & 300.00 & 1024 \\
Garr199904 & reachability & 1280 & 0.03 & 300.00 & 9479 \\
Garr199904 & reachability & 1280 & 0.22 & 300.00 & 1379 \\
Garr199905 & reachability & 1280 & 0.03 & 300.00 & 8973 \\
Garr199905 & reachability & 1280 & 0.21 & 300.00 & 1406 \\
Fccn & reachability & 1292 & 0.03 & 300.00 & 10280 \\
Fccn & reachability & 1292 & 0.26 & 300.00 & 1152 \\
Abvt & reachability & 1316 & 0.10 & 300.00 & 2860 \\
Abvt & reachability & 1316 & 0.33 & 300.00 & 920 \\
Aconet & reachability & 1316 & 0.10 & 300.00 & 3157 \\
Aconet & reachability & 1316 & 0.30 & 300.00 & 991 \\
Renater1999 & reachability & 1365 & 0.04 & 300.00 & 6914 \\
Renater1999 & reachability & 1365 & 0.27 & 300.00 & 1113 \\
VisionNet & reachability & 1365 & 0.04 & 300.00 & 8176 \\
VisionNet & reachability & 1365 & 0.33 & 300.00 & 922 \\
Uran & reachability & 1371 & 0.03 & 300.00 & 9934 \\
Uran & reachability & 1371 & 0.28 & 300.00 & 1090 \\
Psinet & reachability & 1377 & 0.05 & 300.00 & 6153 \\
Psinet & reachability & 1377 & 0.31 & 300.00 & 968 \\
Garr200112 & reachability & 1383 & 0.03 & 300.00 & 10903 \\
Garr200112 & reachability & 1383 & 0.24 & 300.00 & 1245 \\
Belnet2003 & reachability & 1388 & 0.05 & 300.00 & 5907 \\
Belnet2003 & reachability & 1388 & 0.22 & 300.00 & 1355 \\
Belnet2004 & reachability & 1388 & 0.05 & 300.00 & 6007 \\
Belnet2004 & reachability & 1388 & 0.23 & 300.00 & 1289 \\
Renater2001 & reachability & 1389 & 0.05 & 300.00 & 6526 \\
Renater2001 & reachability & 1389 & 0.25 & 300.00 & 1207 \\
Belnet2005 & reachability & 1394 & 0.05 & 300.00 & 5696 \\
Belnet2005 & reachability & 1394 & 0.25 & 300.00 & 1190 \\
Belnet2006 & reachability & 1394 & 0.05 & 300.00 & 6088 \\
Belnet2006 & reachability & 1394 & 0.25 & 300.00 & 1202 \\
Xeex & reachability & 1431 & 0.04 & 300.00 & 6788 \\
Xeex & reachability & 1431 & 0.25 & 300.00 & 1211 \\
BtEurope & reachability & 1449 & 0.05 & 300.00 & 5991 \\
BtEurope & reachability & 1449 & 0.27 & 300.00 & 1128 \\
HurricaneElectric & reachability & 1449 & 0.03 & 300.00 & 9375 \\
HurricaneElectric & reachability & 1449 & 0.24 & 300.00 & 1236 \\
Amres & reachability & 1472 & 0.06 & 300.00 & 4990 \\
Amres & reachability & 1472 & 0.40 & 300.00 & 746 \\
Vinaren & reachability & 1484 & 0.04 & 300.00 & 7723 \\
Vinaren & reachability & 1484 & 0.27 & 300.00 & 1107 \\
Arpanet19723 & reachability & 1496 & 0.07 & 300.00 & 4255 \\
Arpanet19723 & reachability & 1496 & 0.33 & 300.00 & 912 \\
UniC & reachability & 1502 & 0.03 & 300.00 & 8879 \\
UniC & reachability & 1502 & 0.32 & 300.00 & 951 \\
Agis & reachability & 1508 & 0.08 & 300.00 & 3937 \\
Agis & reachability & 1508 & 0.34 & 300.00 & 875 \\
Karen & reachability & 1508 & 0.04 & 300.00 & 6759 \\
Karen & reachability & 1508 & 0.31 & 300.00 & 969 \\
KentmanFeb2008 & reachability & 1601 & 0.05 & 300.00 & 5913 \\
KentmanFeb2008 & reachability & 1601 & 0.30 & 300.00 & 987 \\
Funet & reachability & 1619 & 0.04 & 300.00 & 7503 \\
Funet & reachability & 1619 & 0.36 & 300.00 & 823 \\
AttMpls & reachability & 1670 & 0.05 & 300.00 & 5781 \\
AttMpls & reachability & 1670 & 0.28 & 300.00 & 1085 \\
Bbnplanet & reachability & 1710 & 0.05 & 300.00 & 6151 \\
Bbnplanet & reachability & 1710 & 0.37 & 300.00 & 804 \\
Garr200212 & reachability & 1716 & 0.04 & 300.00 & 8443 \\
Garr200212 & reachability & 1716 & 0.34 & 300.00 & 895 \\
KentmanAug2005 & reachability & 1717 & 0.06 & 300.00 & 5125 \\
KentmanAug2005 & reachability & 1717 & 0.40 & 300.00 & 751 \\
Sunet & reachability & 1727 & 0.04 & 300.00 & 7236 \\
Sunet & reachability & 1727 & 0.37 & 300.00 & 812 \\
Integra & reachability & 1758 & 0.04 & 300.00 & 7486 \\
Integra & reachability & 1758 & 0.33 & 300.00 & 909 \\
Geant2001 & reachability & 1770 & 0.04 & 300.00 & 7857 \\
Geant2001 & reachability & 1770 & 0.32 & 300.00 & 950 \\
Gambia & reachability & 1823 & 0.04 & 300.00 & 7151 \\
Gambia & reachability & 1823 & 0.40 & 300.00 & 747 \\
Darkstrand & reachability & 1841 & 0.07 & 300.00 & 4396 \\
Darkstrand & reachability & 1841 & 0.42 & 300.00 & 717 \\
Shentel & reachability & 1865 & 0.04 & 300.00 & 6725 \\
Shentel & reachability & 1865 & 0.45 & 300.00 & 670 \\
Arpanet19728 & reachability & 1964 & 0.07 & 300.00 & 4560 \\
Arpanet19728 & reachability & 1964 & 0.50 & 300.00 & 604 \\
Biznet & reachability & 1970 & 0.05 & 300.00 & 5705 \\
Biznet & reachability & 1970 & 0.51 & 300.00 & 593 \\
Cesnet200304 & reachability & 1970 & 0.05 & 300.00 & 6618 \\
Cesnet200304 & reachability & 1970 & 0.39 & 300.00 & 762 \\
Janetbackbone & reachability & 2042 & 0.07 & 300.00 & 4073 \\
Janetbackbone & reachability & 2042 & 0.40 & 300.00 & 745 \\
Arn & reachability & 2067 & 0.11 & 300.00 & 2673 \\
Arn & reachability & 2067 & 0.60 & 300.00 & 504 \\
Cynet & reachability & 2067 & 0.07 & 300.00 & 4156 \\
Cynet & reachability & 2067 & 0.47 & 300.00 & 636 \\
GtsHungary & reachability & 2079 & 0.05 & 300.00 & 6003 \\
GtsHungary & reachability & 2079 & 0.55 & 300.00 & 549 \\
Ernet & reachability & 2085 & 0.04 & 300.00 & 6774 \\
Ernet & reachability & 2085 & 0.43 & 300.00 & 690 \\
WideJpn & reachability & 2091 & 0.06 & 300.00 & 5378 \\
WideJpn & reachability & 2091 & 0.42 & 300.00 & 716 \\
Renater2004 & reachability & 2109 & 0.08 & 300.00 & 3736 \\
Renater2004 & reachability & 2109 & 0.45 & 300.00 & 670 \\
Rnp & reachability & 2222 & 0.06 & 300.00 & 5237 \\
Rnp & reachability & 2222 & 0.56 & 300.00 & 536 \\
Iinet & reachability & 2228 & 0.05 & 300.00 & 6191 \\
Iinet & reachability & 2228 & 0.47 & 300.00 & 645 \\
Digex & reachability & 2246 & 0.07 & 300.00 & 4442 \\
Digex & reachability & 2246 & 0.57 & 300.00 & 530 \\
GtsCzechRepublic & reachability & 2345 & 0.05 & 300.00 & 5513 \\
GtsCzechRepublic & reachability & 2345 & 0.61 & 300.00 & 492 \\
DeutscheTelekom & reachability & 2386 & 0.93 & 300.00 & 323 \\
Canerie & reachability & 2393 & 0.05 & 300.00 & 5608 \\
Canerie & reachability & 2393 & 0.55 & 300.00 & 548 \\
GtsPoland & reachability & 2502 & 0.06 & 300.00 & 4997 \\
GtsPoland & reachability & 2502 & 0.65 & 300.00 & 462 \\
CrlNetworkServices & reachability & 2508 & 0.09 & 300.00 & 3349 \\
CrlNetworkServices & reachability & 2508 & 0.59 & 300.00 & 512 \\
IowaStatewideFiberMap & reachability & 2526 & 0.06 & 300.00 & 5046 \\
IowaStatewideFiberMap & reachability & 2526 & 0.63 & 300.00 & 475 \\
Renater2006 & reachability & 2538 & 0.08 & 300.00 & 3629 \\
Renater2006 & reachability & 2538 & 0.55 & 300.00 & 546 \\
Renater2008 & reachability & 2538 & 0.06 & 300.00 & 4812 \\
Renater2008 & reachability & 2538 & 0.57 & 300.00 & 531 \\
Bics & reachability & 2568 & 0.06 & 300.00 & 4688 \\
Bics & reachability & 2568 & 0.57 & 300.00 & 526 \\
Arnes & reachability & 2699 & 0.14 & 300.00 & 2168 \\
Arnes & reachability & 2699 & 0.78 & 300.00 & 384 \\
Xspedius & reachability & 2711 & 0.08 & 300.00 & 3604 \\
Xspedius & reachability & 2711 & 0.59 & 300.00 & 511 \\
Geant2009 & reachability & 2729 & 0.07 & 300.00 & 4252 \\
Geant2009 & reachability & 2729 & 0.58 & 300.00 & 519 \\
Zamren & reachability & 2763 & 0.07 & 300.00 & 4142 \\
Zamren & reachability & 2763 & 0.83 & 300.00 & 359 \\
GtsSlovakia & reachability & 2780 & 0.06 & 300.00 & 4845 \\
GtsSlovakia & reachability & 2780 & 0.73 & 300.00 & 412 \\
NetworkUsa & reachability & 2792 & 0.11 & 300.00 & 2824 \\
NetworkUsa & reachability & 2792 & 0.77 & 300.00 & 391 \\
Cwix & reachability & 2949 & 0.10 & 300.00 & 2933 \\
Cwix & reachability & 2949 & 0.77 & 300.00 & 392 \\
Niif & reachability & 2949 & 0.11 & 300.00 & 2809 \\
Niif & reachability & 2949 & 0.69 & 300.00 & 433 \\
PionierL1 & reachability & 2949 & 0.10 & 300.00 & 2893 \\
PionierL1 & reachability & 2949 & 0.75 & 300.00 & 397 \\
Reuna & reachability & 3068 & 0.16 & 300.00 & 1833 \\
Reuna & reachability & 3068 & 0.86 & 300.00 & 347 \\
Bren & reachability & 3080 & 0.08 & 300.00 & 3568 \\
Bren & reachability & 3080 & 0.75 & 300.00 & 401 \\
Myren & reachability & 3092 & 0.10 & 300.00 & 3003 \\
Myren & reachability & 3092 & 0.69 & 300.00 & 432 \\
Evolink & reachability & 3122 & 0.08 & 300.00 & 3756 \\
Evolink & reachability & 3122 & 0.88 & 300.00 & 341 \\
Grnet & reachability & 3134 & 0.07 & 300.00 & 4325 \\
Grnet & reachability & 3134 & 0.76 & 300.00 & 395 \\
BtNorthAmerica & reachability & 3159 & 0.09 & 300.00 & 3430 \\
BtNorthAmerica & reachability & 3159 & 0.67 & 300.00 & 450 \\
Geant2010 & reachability & 3200 & 0.08 & 300.00 & 3759 \\
Geant2010 & reachability & 3200 & 0.72 & 300.00 & 416 \\
KentmanJan2011 & reachability & 3239 & 0.10 & 300.00 & 2967 \\
KentmanJan2011 & reachability & 3239 & 0.82 & 300.00 & 366 \\
Iij & reachability & 3248 & 0.08 & 300.00 & 3673 \\
Iij & reachability & 3248 & 0.80 & 300.00 & 377 \\
PionierL3 & reachability & 3317 & 0.12 & 300.00 & 2458 \\
PionierL3 & reachability & 3317 & 0.85 & 300.00 & 352 \\
Cesnet200511 & reachability & 3426 & 0.08 & 300.00 & 3776 \\
Cesnet200511 & reachability & 3426 & 0.85 & 300.00 & 354 \\
Cesnet200603 & reachability & 3426 & 0.09 & 300.00 & 3509 \\
Cesnet200603 & reachability & 3426 & 0.87 & 300.00 & 344 \\
Ntt & reachability & 3458 & 0.17 & 300.00 & 1745 \\
Ntt & reachability & 3458 & 1.13 & 300.00 & 265 \\
Intranetwork & reachability & 3480 & 0.10 & 300.00 & 3033 \\
Intranetwork & reachability & 3480 & 1.12 & 300.00 & 269 \\
Geant2012 & reachability & 3689 & 0.09 & 300.00 & 3392 \\
Geant2012 & reachability & 3689 & 0.90 & 300.00 & 332 \\
Cernet & reachability & 3842 & 0.13 & 300.00 & 2346 \\
Cernet & reachability & 3842 & 0.97 & 300.00 & 309 \\
LambdaNet & reachability & 3933 & 0.15 & 300.00 & 1964 \\
LambdaNet & reachability & 3933 & 1.38 & 300.00 & 217 \\
Roedunet & reachability & 3957 & 0.09 & 300.00 & 3176 \\
Roedunet & reachability & 3957 & 1.08 & 300.00 & 279 \\
SwitchL3 & reachability & 4035 & 0.10 & 300.00 & 3058 \\
SwitchL3 & reachability & 4035 & 0.95 & 300.00 & 315 \\
Chinanet & reachability & 4053 & 0.16 & 300.00 & 1888 \\
Chinanet & reachability & 4053 & 1.03 & 300.00 & 293 \\
Litnet & reachability & 4088 & 0.12 & 300.00 & 2449 \\
Litnet & reachability & 4088 & 0.99 & 300.00 & 303 \\
Sanet & reachability & 4100 & 0.10 & 300.00 & 3014 \\
Sanet & reachability & 4100 & 1.35 & 300.00 & 222 \\
Renater2010 & reachability & 4166 & 0.10 & 300.00 & 2976 \\
Renater2010 & reachability & 4166 & 1.15 & 300.00 & 261 \\
Carnet & reachability & 4265 & 0.10 & 300.00 & 2919 \\
Carnet & reachability & 4265 & 1.33 & 300.00 & 225 \\
Cesnet200706 & reachability & 4313 & 0.10 & 300.00 & 3028 \\
Cesnet200706 & reachability & 4313 & 1.15 & 300.00 & 261 \\
BtLatinAmerica & reachability & 4494 & 0.09 & 300.00 & 3182 \\
BtLatinAmerica & reachability & 4494 & 1.99 & 300.00 & 150 \\
Palmetto & reachability & 4608 & 0.17 & 300.00 & 1764 \\
Palmetto & reachability & 4608 & 1.33 & 300.00 & 226 \\
Ntelos & reachability & 4929 & 0.18 & 300.00 & 1687 \\
Ntelos & reachability & 4929 & 1.84 & 300.00 & 163 \\
RoedunetFibre & reachability & 5067 & 0.13 & 300.00 & 2359 \\
RoedunetFibre & reachability & 5067 & 1.60 & 300.00 & 188 \\
Bellcanada & reachability & 5145 & 0.17 & 300.00 & 1788 \\
Bellcanada & reachability & 5145 & 1.69 & 300.00 & 177 \\
Uunet & reachability & 5456 & 0.18 & 300.00 & 1661 \\
Uunet & reachability & 5456 & 1.43 & 300.00 & 209 \\
Surfnet & reachability & 5591 & 0.14 & 300.00 & 2165 \\
Surfnet & reachability & 5591 & 1.70 & 300.00 & 176 \\
Cudi & reachability & 5670 & 0.18 & 300.00 & 1663 \\
Cudi & reachability & 5670 & 1.63 & 300.00 & 184 \\
Iris & reachability & 5742 & 0.19 & 300.00 & 1580 \\
Iris & reachability & 5742 & 1.90 & 300.00 & 158 \\
Bellsouth & reachability & 5754 & 0.22 & 300.00 & 1368 \\
Bellsouth & reachability & 5754 & 1.98 & 300.00 & 152 \\
Cesnet201006 & reachability & 5945 & 0.23 & 300.00 & 1284 \\
Cesnet201006 & reachability & 5945 & 1.85 & 300.00 & 162 \\
BeyondTheNetwork & reachability & 6170 & 0.14 & 300.00 & 2160 \\
BeyondTheNetwork & reachability & 6170 & 1.83 & 300.00 & 164 \\
Tinet & reachability & 6314 & 0.16 & 300.00 & 1887 \\
Tinet & reachability & 6314 & 1.83 & 300.00 & 164 \\
Garr200908 & reachability & 6405 & 0.14 & 300.00 & 2092 \\
Garr200908 & reachability & 6405 & 1.86 & 300.00 & 161 \\
Garr200912 & reachability & 6405 & 0.15 & 300.00 & 1965 \\
Garr200912 & reachability & 6405 & 1.91 & 300.00 & 157 \\
Garr201001 & reachability & 6405 & 0.14 & 300.00 & 2077 \\
Garr201001 & reachability & 6405 & 1.84 & 300.00 & 163 \\
Garr200902 & reachability & 6423 & 0.14 & 300.00 & 2074 \\
Garr200902 & reachability & 6423 & 1.81 & 300.00 & 166 \\
Garr201003 & reachability & 6423 & 0.15 & 300.00 & 2066 \\
Garr201003 & reachability & 6423 & 1.85 & 300.00 & 162 \\
Garr201004 & reachability & 6423 & 0.15 & 300.00 & 2040 \\
Garr201004 & reachability & 6423 & 1.88 & 300.00 & 159 \\
Garr200909 & reachability & 6632 & 0.17 & 300.00 & 1771 \\
Garr200909 & reachability & 6632 & 2.02 & 300.00 & 148 \\
Garr201005 & reachability & 6650 & 0.16 & 300.00 & 1929 \\
Garr201005 & reachability & 6650 & 1.96 & 300.00 & 153 \\
Garr201007 & reachability & 6662 & 0.15 & 300.00 & 2037 \\
Garr201007 & reachability & 6662 & 1.89 & 300.00 & 158 \\
Garr201008 & reachability & 6662 & 0.15 & 300.00 & 2016 \\
Garr201008 & reachability & 6662 & 1.89 & 300.00 & 158 \\
HiberniaGlobal & reachability & 6704 & 0.16 & 300.00 & 1903 \\
HiberniaGlobal & reachability & 6704 & 2.53 & 300.00 & 119 \\
Garr201010 & reachability & 6893 & 0.15 & 300.00 & 1986 \\
Garr201010 & reachability & 6893 & 2.01 & 300.00 & 149 \\
Garr201012 & reachability & 6893 & 0.15 & 300.00 & 1973 \\
Garr201012 & reachability & 6893 & 2.01 & 300.00 & 149 \\
Garr201101 & reachability & 6899 & 0.16 & 300.00 & 1918 \\
Garr201101 & reachability & 6899 & 2.07 & 300.00 & 145 \\
Garr201102 & reachability & 7134 & 0.16 & 300.00 & 1873 \\
Garr201102 & reachability & 7134 & 2.19 & 300.00 & 137 \\
Garr201103 & reachability & 7391 & 0.17 & 300.00 & 1776 \\
Garr201103 & reachability & 7391 & 2.46 & 300.00 & 122 \\
Dfn & reachability & 7427 & 0.23 & 300.00 & 1309 \\
Dfn & reachability & 7427 & 2.65 & 300.00 & 113 \\
Garr201104 & reachability & 7640 & 0.20 & 300.00 & 1474 \\
Garr201104 & reachability & 7640 & 2.37 & 300.00 & 127 \\
Garr201105 & reachability & 7646 & 0.18 & 300.00 & 1676 \\
Garr201105 & reachability & 7646 & 2.36 & 300.00 & 127 \\
Garr201107 & reachability & 7652 & 0.17 & 300.00 & 1721 \\
Garr201107 & reachability & 7652 & 2.32 & 300.00 & 129 \\
Garr201108 & reachability & 7652 & 0.17 & 300.00 & 1746 \\
Garr201108 & reachability & 7652 & 2.36 & 300.00 & 127 \\
Garr201109 & reachability & 7658 & 0.17 & 300.00 & 1760 \\
Garr201109 & reachability & 7658 & 2.47 & 300.00 & 121 \\
Garr201110 & reachability & 7664 & 0.17 & 300.00 & 1725 \\
Garr201110 & reachability & 7664 & 2.51 & 300.00 & 120 \\
Garr201111 & reachability & 7905 & 0.18 & 300.00 & 1626 \\
Garr201111 & reachability & 7905 & 2.62 & 300.00 & 115 \\
UsSignal & reachability & 8104 & 0.25 & 300.00 & 1218 \\
UsSignal & reachability & 8104 & 3.29 & 300.00 & 91 \\
Garr201112 & reachability & 8162 & 0.19 & 300.00 & 1600 \\
Garr201112 & reachability & 8162 & 2.70 & 300.00 & 111 \\
Garr201201 & reachability & 8162 & 0.19 & 300.00 & 1581 \\
Garr201201 & reachability & 8162 & 2.53 & 300.00 & 119 \\
Forthnet & reachability & 8249 & 0.18 & 300.00 & 1712 \\
Forthnet & reachability & 8249 & 3.18 & 300.00 & 94 \\
AsnetAm & reachability & 9122 & 0.26 & 300.00 & 1151 \\
AsnetAm & reachability & 9122 & 3.60 & 300.00 & 83 \\
Internode & reachability & 9381 & 0.19 & 300.00 & 1553 \\
Internode & reachability & 9381 & 3.06 & 300.00 & 98 \\
Missouri & reachability & 9680 & 0.34 & 300.00 & 883 \\
Missouri & reachability & 9680 & 3.86 & 300.00 & 78 \\
Globenet & reachability & 9860 & 0.23 & 300.00 & 1313 \\
Globenet & reachability & 9860 & 3.70 & 300.00 & 81 \\
Esnet & reachability & 10007 & 0.22 & 300.00 & 1349 \\
Esnet & reachability & 10007 & 3.90 & 300.00 & 77 \\
Latnet & reachability & 10176 & 0.39 & 300.00 & 776 \\
Latnet & reachability & 10176 & 5.04 & 300.00 & 60 \\
Uninett2011 & reachability & 10320 & 0.25 & 300.00 & 1193 \\
Uninett2011 & reachability & 10320 & 3.52 & 300.00 & 85 \\
Columbus & reachability & 10523 & 0.28 & 300.00 & 1076 \\
Columbus & reachability & 10523 & 4.64 & 300.00 & 65 \\
Telcove & reachability & 10720 & 0.23 & 300.00 & 1315 \\
Telcove & reachability & 10720 & 4.43 & 300.00 & 68 \\
Tw & reachability & 11011 & 0.28 & 300.00 & 1090 \\
Tw & reachability & 11011 & 4.23 & 300.00 & 71 \\
Intellifiber & reachability & 11462 & 0.27 & 300.00 & 1104 \\
Intellifiber & reachability & 11462 & 4.82 & 300.00 & 62 \\
Syringa & reachability & 11621 & 0.35 & 300.00 & 864 \\
Syringa & reachability & 11621 & 7.58 & 300.00 & 40 \\
Sinet & reachability & 11633 & 0.25 & 300.00 & 1183 \\
Sinet & reachability & 11633 & 4.39 & 300.00 & 68 \\
Switch & reachability & 11729 & 0.28 & 300.00 & 1073 \\
Switch & reachability & 11729 & 5.02 & 300.00 & 60 \\
Uninett2010 & reachability & 11783 & 0.27 & 300.00 & 1105 \\
Uninett2010 & reachability & 11783 & 4.17 & 300.00 & 72 \\
Ulaknet & reachability & 14189 & 0.43 & 300.00 & 690 \\
Ulaknet & reachability & 14189 & 12.73 & 300.00 & 24 \\
Oteglobe & reachability & 14724 & 8.56 & 300.00 & 35 \\
RedBestel & reachability & 14973 & 0.57 & 300.00 & 525 \\
RedBestel & reachability & 14973 & 9.47 & 300.00 & 32 \\
VtlWavenet2008 & reachability & 16307 & 0.66 & 300.00 & 457 \\
VtlWavenet2008 & reachability & 16307 & 11.72 & 300.00 & 26 \\
VtlWavenet2011 & reachability & 17783 & 0.71 & 300.00 & 421 \\
VtlWavenet2011 & reachability & 17783 & 13.04 & 300.00 & 23 \\
Interoute & reachability & 25475 & 0.65 & 300.00 & 464 \\
Interoute & reachability & 25475 & 14.66 & 300.00 & 20 \\
Deltacom & reachability & 26978 & 1.10 & 300.00 & 273 \\
Deltacom & reachability & 26978 & 17.03 & 300.00 & 18 \\
Ion & reachability & 32528 & 0.98 & 300.00 & 305 \\
Ion & reachability & 32528 & 24.15 & 300.00 & 12 \\
Pern & reachability & 33416 & 1.11 & 300.00 & 270 \\
Pern & reachability & 33416 & 21.70 & 300.00 & 14 \\
DialtelecomCz & reachability & 39466 & 1.23 & 300.00 & 244 \\
DialtelecomCz & reachability & 39466 & 62.13 & 300.00 & 5 \\
TataNld & reachability & 43652 & 1.28 & 300.00 & 234 \\
TataNld & reachability & 43652 & 32.92 & 300.00 & 9 \\
GtsCe & reachability & 46010 & 1.47 & 300.00 & 203 \\
GtsCe & reachability & 46010 & 34.82 & 300.00 & 9 \\
Colt & reachability & 48426 & 1.66 & 300.00 & 181 \\
Colt & reachability & 48426 & 37.43 & 300.00 & 8 \\
UsCarrier & reachability & 51539 & 1.71 & 300.00 & 176 \\
UsCarrier & reachability & 51539 & 45.41 & 300.00 & 7 \\
Cogentco & reachability & 79682 & 2.61 & 300.00 & 115 \\
Cogentco & reachability & 79682 & 77.62 & 300.00 & 4 \\
\bottomrule
\end{tabular}


==> plots/Inc_comparison_table.tex <==
\begin{tabular}{lrrrr}
\toprule
Name & Size (KB) & KATch (s) & Frenetic (s) & Speedup \\
\midrule
inc1 & 0.31 & 0.07 & 0.04 & 1 \\
inc2 & 0.56 & 0.00 & 0.03 & 13 \\
inc3 & 0.81 & 0.00 & 0.03 & 11 \\
inc4 & 1.06 & 0.00 & 0.04 & 11 \\
inc5 & 1.30 & 0.00 & 0.06 & 13 \\
inc6 & 1.55 & 0.01 & 0.19 & 34 \\
inc7 & 1.80 & 0.01 & 1.02 & 140 \\
inc8 & 2.05 & 0.01 & 7.78 & 970 \\
inc9 & 2.30 & 0.01 & 67.95 & 7459 \\
inc10 & 2.56 & 0.04 & 586.50 & 13229 \\
\bottomrule
\end{tabular}


==> plots/Inc_comparison_table_old.tex <==
\begin{tabular}{lrrrr}
\toprule
Name & Size & KATch (s) & Frenetic (s) & Speedup \\
\midrule
inc1 & 23 & 0.07 & 0.04 & 1 \\
inc2 & 42 & 0.00 & 0.03 & 13 \\
inc3 & 61 & 0.00 & 0.03 & 11 \\
inc4 & 80 & 0.00 & 0.04 & 11 \\
inc5 & 99 & 0.00 & 0.06 & 13 \\
inc6 & 118 & 0.01 & 0.19 & 34 \\
inc7 & 137 & 0.01 & 1.02 & 140 \\
inc8 & 156 & 0.01 & 7.78 & 970 \\
inc9 & 175 & 0.01 & 67.95 & 7459 \\
inc10 & 194 & 0.04 & 586.50 & 13229 \\
\bottomrule
\end{tabular}


==> plots/Non-determinism_comparison_table.tex <==
\begin{tabular}{lrrrr}
\toprule
Name & Size (KB) & KATch (s) & Frenetic (s) & Speedup \\
\midrule
nondet1 & 0.13 & 0.00 & 0.03 & 15 \\
nondet2 & 0.17 & 0.00 & 0.03 & 16 \\
nondet3 & 0.21 & 0.00 & 0.04 & 20 \\
nondet4 & 0.24 & 0.00 & 0.08 & 40 \\
nondet5 & 0.28 & 0.00 & 0.17 & 69 \\
nondet6 & 0.32 & 0.00 & 0.37 & 145 \\
nondet7 & 0.36 & 0.00 & 0.83 & 304 \\
nondet8 & 0.39 & 0.00 & 1.77 & 563 \\
nondet9 & 0.43 & 0.00 & 3.28 & 939 \\
nondet10 & 0.47 & 0.01 & 5.84 & 1077 \\
nondet11 & 0.51 & 0.01 & 9.71 & 1619 \\
nondet12 & 0.55 & 0.01 & 15.77 & 2287 \\
nondet13 & 0.59 & 0.01 & 24.80 & 3353 \\
nondet14 & 0.63 & 0.01 & 37.81 & 4054 \\
nondet15 & 0.67 & 0.01 & 54.60 & 5344 \\
\bottomrule
\end{tabular}


==> plots/Nondet_comparison_table.tex <==
\begin{tabular}{lrrrr}
\toprule
Name & Size (KB) & KATch (s) & Frenetic (s) & Speedup \\
\midrule
nondet1 & 0.13 & 0.00 & 0.03 & 15 \\
nondet2 & 0.17 & 0.00 & 0.03 & 16 \\
nondet3 & 0.21 & 0.00 & 0.04 & 20 \\
nondet4 & 0.24 & 0.00 & 0.08 & 40 \\
nondet5 & 0.28 & 0.00 & 0.17 & 69 \\
nondet6 & 0.32 & 0.00 & 0.37 & 145 \\
nondet7 & 0.36 & 0.00 & 0.83 & 304 \\
nondet8 & 0.39 & 0.00 & 1.77 & 563 \\
nondet9 & 0.43 & 0.00 & 3.28 & 939 \\
nondet10 & 0.47 & 0.01 & 5.84 & 1077 \\
nondet11 & 0.51 & 0.01 & 9.71 & 1619 \\
nondet12 & 0.55 & 0.01 & 15.77 & 2287 \\
nondet13 & 0.59 & 0.01 & 24.80 & 3353 \\
nondet14 & 0.63 & 0.01 & 37.81 & 4054 \\
nondet15 & 0.67 & 0.01 & 54.60 & 5344 \\
\bottomrule
\end{tabular}


==> plots/Nondet_comparison_table_old.tex <==
\begin{tabular}{lrrrr}
\toprule
Name & Size & KATch (s) & Frenetic (s) & Speedup \\
\midrule
nondet1 & 10 & 0.00 & 0.03 & 15 \\
nondet2 & 13 & 0.00 & 0.03 & 16 \\
nondet3 & 16 & 0.00 & 0.04 & 20 \\
nondet4 & 19 & 0.00 & 0.08 & 40 \\
nondet5 & 22 & 0.00 & 0.17 & 69 \\
nondet6 & 25 & 0.00 & 0.37 & 145 \\
nondet7 & 28 & 0.00 & 0.83 & 304 \\
nondet8 & 31 & 0.00 & 1.77 & 563 \\
nondet9 & 34 & 0.00 & 3.28 & 939 \\
nondet10 & 37 & 0.01 & 5.84 & 1077 \\
nondet11 & 40 & 0.01 & 9.71 & 1619 \\
nondet12 & 43 & 0.01 & 15.77 & 2287 \\
nondet13 & 46 & 0.01 & 24.80 & 3353 \\
nondet14 & 49 & 0.01 & 37.81 & 4054 \\
nondet15 & 52 & 0.01 & 54.60 & 5344 \\
\bottomrule
\end{tabular}

